Draw and Tell: Teaching Text-to-Image Diffusion Models to Describe What They Draw

Text-to-image (T2I) diffusion models read text and generate images, but they never write. We present Draw-and-Tell, which makes a pre-trained T2I model also write what it draws. Alongside the image, the model co-generates a description of it as a stream of text-encoder states, denoised by the same rectified flow, and a one-layer language-model read-out turns the stream into words. The backbone is adapted with LoRA, and text-only MLPs give the description capacity of its own. The description works like a representation-alignment target that the backbone must write rather than only match: during training it shapes the weights the image is drawn with, and the image itself never reads it. With minimal resources, 13M text tokens and about 17 GH200 GPU-hours, the model can be made to write: on SD3.5 Medium and FLUX.2 [klein], its descriptions of held-out prompts are read back at a perplexity of 46 and 26. And it draws better: GenEval rises from 68.4 to 74.3 on SD3.5 and from 76.3 to 79.0 on FLUX.2 [klein], above a matched image-only fine-tuning control (73.4 and 77.2), and the gain comes from writing, not from aligning to or training on the descriptions. Blind MLLM judges prefer its images to the control's for fine detail (56% and 60% of decided pairs), and a user study confirms this. The judges also find that, on short, ambiguous prompts, it commits to a meaningful reading of the prompt. With the description switched off, the network keeps the original architecture and inference cost, with fine-tuned weights.

==> fig/src/figstyle.tex <==
% Shared style for all TikZ / pgfplots figures (Times, to match cvpr.sty).
% One palette, defined once: edit the block below and re-run build.sh to restyle every figure.
\usepackage{times}
\usepackage{amsmath,amssymb}
\usepackage{pifont}
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=1.18}
\usetikzlibrary{positioning,calc,fit,arrows.meta,patterns,shapes.misc,backgrounds,decorations.pathreplacing}
\usepgfplotslibrary{groupplots}

% ---- palette (light): ColorBrewer RdBu tones
\definecolor{ink}{HTML}{222222}        % text
\definecolor{outline}{HTML}{6E6E6E}    % box outlines, arrows
\definecolor{muted}{HTML}{666666}      % secondary text
\definecolor{rule}{HTML}{BDBDBD}       % grid, frozen outlines
\definecolor{light}{HTML}{EFEFEF}      % caption tokens, "equal" bars
\definecolor{mid}{HTML}{D6D6D6}
\definecolor{accent}{HTML}{D6604D}     % words / description stream / ours: lines and text
\definecolor{accentbar}{HTML}{F4A582}  % ... bars and fills
\definecolor{tint}{HTML}{FDDBC7}       % description tokens
\definecolor{pix}{HTML}{4393C3}        % pixels / image pathway: lines and text
\definecolor{pixbar}{HTML}{92C5DE}     % ... bars
\definecolor{pixtint}{HTML}{D1E5F0}    % image latent tokens
\definecolor{dark}{HTML}{4393C3}       % second series in line charts
\definecolor{basecol}{HTML}{BABABA}    % base model / opponent in charts
\definecolor{sftcol}{HTML}{8C8C8C}     % SFT control in line charts
\definecolor{todo}{HTML}{C8102E}

\newcommand{\fsz}{\fontsize{6}{7}\selectfont}
\newcommand{\fsx}{\fontsize{5.5}{6.5}\selectfont}
\tikzset{
  every node/.style={font=\scriptsize, text=ink},
  box/.style={draw=outline, line width=0.5pt, rounded corners=2pt, fill=white, inner xsep=4pt, inner ysep=3pt, align=center},
  greybox/.style={box, draw=rule, fill=light!60},
  accentbox/.style={box, draw=accent, fill=tint!55, line width=0.7pt},
  pixbox/.style={box, draw=pix, fill=pixtint!55, line width=0.6pt},
  lab/.style={font=\fsz, text=muted, align=center, inner sep=1pt},
  lab7/.style={font=\scriptsize, text=muted, align=center, inner sep=1pt},
  tlab/.style={font=\bfseries\footnotesize, text=ink, inner sep=1pt, align=left},
  arr/.style={-{Stealth[length=4pt,width=3.2pt]}, line width=0.55pt, draw=outline},
  aarr/.style={-{Stealth[length=4pt,width=3.2pt]}, line width=0.7pt, draw=accent},
  parr/.style={-{Stealth[length=4pt,width=3.2pt]}, line width=0.7pt, draw=pix},
  adash/.style={-{Stealth[length=4pt,width=3.2pt]}, line width=0.7pt, draw=accent, dash pattern=on 2.5pt off 1.5pt},
  thin/.style={line width=0.4pt, draw=outline},
}

% token rows:  \tokrow{x}{y}{n}{fill}{line}{hatch 0/1}
\newlength{\tokside}\setlength{\tokside}{0.2cm}
\newcommand{\tokrow}[6]{%
  \foreach \i in {0,...,\numexpr#3-1\relax} {%
    \fill[#4] ({#1+\i*0.25},#2) rectangle ++(\tokside,\tokside);
    \ifnum#6=1 \path[pattern=north east lines, pattern color=#5!75] ({#1+\i*0.25},#2) rectangle ++(\tokside,\tokside);\fi
    \draw[#5, line width=0.35pt] ({#1+\i*0.25},#2) rectangle ++(\tokside,\tokside);
  }%
}

% ---- pgfplots house style
\pgfplotsset{
  house/.style={
    axis line style={rule, line width=0.4pt},
    tick style={rule, line width=0.3pt},
    tick label style={font=\fsz, text=muted},
    label style={font=\fsz, text=muted},
    title style={font=\scriptsize\bfseries, text=ink, at={(0,1)}, anchor=south west, yshift=1pt},
    legend style={draw=none, fill=none, font=\fsz, legend cell align=left, row sep=-1pt, column sep=4pt},
    grid style={rule!45, line width=0.3pt},
  },
  % stacked horizontal preference bars: ours | equal | opponent
  prefbars/.style={
    house,
    xbar stacked, bar width=7pt, xmin=0, xmax=100,
    xtick={0,25,50,75,100}, xticklabels={0,25,50,75,100\%},
    axis x line*=bottom, axis y line*=left, ytick style={draw=none},
    yticklabel style={font=\fsz, text=ink},
    enlarge y limits=0.22,
    nodes near coords, nodes near coords style={font=\fsx, text=ink},
    nodes near coords align={center},
    point meta=rawx,
    every axis plot/.append style={draw=white, line width=0.4pt},
  },
}
% a vertical 50% reference line inside an axis
\newcommand{\parityline}{\draw[muted, dashed, line width=0.5pt] (rel axis cs:0.5,0) -- (rel axis cs:0.5,1);}

